Sampling with Mollified Interaction Energy Descent

Sampling from a target measure whose density is only known up to a normalization constant is a fundamental problem in computational statistics and machine learning. In this paper, we present a new optimization-based method for sampling called mollified interaction energy descent (MIED). MIED minimizes a new class of energies on probability measures called mollified interaction energies (MIEs). These energies rely on mollifier functions -- smooth approximations of the Dirac delta originated from PDE theory. We show that as the mollifier approaches the Dirac delta, the MIE converges to the chi-square divergence with respect to the target measure and the gradient flow of the MIE agrees with that of the chi-square divergence. Optimizing this energy with proper discretization yields a practical first-order particle-based algorithm for sampling in both unconstrained and constrained domains. We show experimentally that for unconstrained sampling problems our algorithm performs on par with existing particle-based algorithms like SVGD, while for constrained sampling problems our method readily incorporates constrained optimization techniques to handle more flexible constraints with strong performance compared to alternatives.

==> analysis.tex <==
\section{Analysis of the full-dimensional case}
\lingxiao{A more careful/general version is in the appendix.}

We analyze the gradient flow of the proposed energy in the full dimension, i.e., $d = n$.
All integration will be over $\RR^n$ if unspecified.
Let $p(x): \RR^n \to \RR_{\ge 0}$ be the (unnormalized) target density that we hope to sample from.
In this section we assume $s > n$.
Define for $\epsilon > 0$, the \emph{regularized Riesz kernel} (also known as \emph{the inverse multi-quadratic kernel}).
\begin{align}\label{eqn:reg_riesz_kernel}
  k_{\epsilon}(x, y) \defeq \frac{1}{(\norm{x-y}^2_2 + \epsilon^2)^{s/2}}.
\end{align}
\lingxiao{An alternative choice of kernel is $(\norm{x-y}^2+\epsilon^2)^{-(s/2+1)}\norm{x-y}$. The benefit is then we don't need to add the diagonal term --- this agrees with the discrete algorithm more. I believe the theory still goes through --- the only thing we need from the kernel is the convergence of convolution.}
Then $k_{\epsilon}$ is an integrable positive definite kernel since $s > n$.
Let 
\begin{align}
  I_{\epsilon} \defeq \int k_\epsilon(0, x) \dd x < \infty
\end{align}
be the normalizing constant.
Define the normalized version of \eqref{eqn:reg_riesz_kernel} as
\begin{align}\label{eqn:normalized_reg_riesz_kernel}
  \hat{k}_{\epsilon}(x, y) \defeq k_\epsilon(x,y) / I_\epsilon.
\end{align}

Next we establish a few bounds for integration with $k_\epsilon$.
\begin{lemma}\label{lem:kernel_int}
  Let $b \ge 0$.
  Then for any $\epsilon > 0$, 
  \begin{align}\label{eqn:kernel_int_eq}
    \int_{B_\epsilon(0)} k_\epsilon(0, y) \norm{y}_2^b \dd y =
    \mathcal{H}_{n-1}(S^{n-1})\left( \int_0^1 \frac{t^{n+b-1}}{(t^2+1)^{s/2}} \right)\epsilon^{n+b-s},
  \end{align}
  where $\mathcal{H}_{n-1}(S^{n-1})$ is the volume of the $(n-1)$-dimensional sphere.

  Furthermore, assuming $s > b + n$, then for any $\epsilon > 0, \delta > 0$,
  \begin{align}
    \int_{\RR^n \setminus B_\delta(0)} k_\epsilon(0, y) \norm{y}_2^b \dd y  
    &\le \mathcal{H}_{n-1}(S^{n-1})\frac{\delta^{n+b-s}}{s-(n+b)} .\label{eqn:kernel_int_complement_ub}
  \end{align}
\end{lemma}
\begin{proof}
  For \eqref{eqn:kernel_int_eq}, we compute
  \begin{align*}
    \int_{B_\epsilon(0)} k_\epsilon(0, y) \norm{y}_2^b \dd y &= \int_{B_\epsilon(0)}\frac{\norm{y}_2^b}{(\norm{y}_2^2+\epsilon^2)^{s/2}} =
\mathcal{H}_{n-1}(S^{n-1})\int_0^\epsilon \frac{r^{n+b-1}}{(r^2+\epsilon^2)^{s/2}} \dd r \\
                                                             &= \mathcal{H}_{n-1}(S^{n-1})\int_0^1 \frac{(\epsilon t)^{n+b - 1}}{(\epsilon^2 t^2 + \epsilon^2)^{s/2}} \epsilon \dd t \\
                                                             &= \mathcal{H}_{n-1}(S^{n-1})\left(\int_0^1 \frac{t^{n+b - 1}}{(t^2+1)^{s/2}}\dd t\right)\epsilon^{n+b-s},
  \end{align*}
  where we use substitution $r = \epsilon t$ on the second line.

  If $s > b + n$, then
  \begin{align*}
    \int_{\RR^n \setminus B_\delta(0)} k_\epsilon(0, y) \norm{y}_2^b \dd y &= \int_{\RR^n \setminus B_\delta(0)} \frac{\norm{y}_2^b}{(\norm{y}_2^2+\epsilon^2)^{s/2}}  \\
                                                                           &\le \int_{\RR^n \setminus B_\delta(0)} \frac{\norm{y}_2^b}{\norm{y}_2^s} = \mathcal{H}_{n-1}(S^{n-1})\int_\delta^\infty r^{n-1+b-s}  \\
                                                                           &= \mathcal{H}_{n-1}(S^{n-1}) \frac{\delta^{n+b-s}}{s-(n+b)},
  \end{align*}
  where the last integral uses $s > b + n$.
\end{proof}

\begin{proposition}\label{prop:kernel_measure_conv_delta}
  Assume $s > n$.
  Define $\nu_\epsilon$ to be the probability measure 
  \begin{align}\label{eqn:riesz_kernel_measure}
   \nu_\epsilon(x) = \hat{k}_\epsilon(0, x) \dd x.
  \end{align}
  Then $\nu_\epsilon$ converges in probability to $\delta_0$, the point measure at $0$.
\end{proposition}
\begin{proof}
  For any $\delta > 0$, we have for $\epsilon < \delta$,
  \begin{align*}
    \nu_\epsilon(B_\delta(0)) &= \int_{B_\delta(0)} \hat{k}_\epsilon(0, x) \dd x 
                              = \frac{\int_{B_\delta(0)}k_\epsilon(0,x)\dd x}{I_\epsilon}
                              \ge \frac{\int_{B_\epsilon(0)} k_\epsilon(0, x) \dd x}{I_\epsilon} = C \epsilon^{n-s}/I_\epsilon,
  \end{align*}
  where we use \eqref{eqn:kernel_int_eq} with $b = 0$ and $C$ is a constant depending only on $n, s$.
  On the other hand, by \eqref{eqn:kernel_int_complement_ub} with $b = 0$,
  \begin{align*}
    \nu_\epsilon(\RR^n \setminus B_\delta(0)) = \frac{\int_{\RR^n \setminus B_\delta(0)}k_\epsilon(0,x)\dd x}{I_\epsilon} \le C' \delta^{n-s} / I_\epsilon.
  \end{align*}
  Since $\delta$ is fixed and $s > n$, we see that
  \[
    \lim_{\epsilon \to 0} \frac{\nu_\epsilon(B_\delta(0))}{\nu_\epsilon(\RR^n \setminus B_\delta(0))} = \lim_{\epsilon \to 0} \frac{C\epsilon^{n-s}}{C'\delta^{n-s}} = \infty
  .\]
  Hence
  \begin{align*}
    \lim_{\epsilon \to 0} \nu_\epsilon(\RR^n \setminus B_\delta(0)) &= \lim_{\epsilon \to 0} \frac{\nu_\epsilon(\RR^n \setminus B_\delta(0))}{\nu_\epsilon(B_\delta(0)) + \nu_\epsilon(\RR^n \setminus B_\delta(0))} 
                                                                    = \lim_{\epsilon \to 0} \frac{1}{\frac{\nu_\epsilon(B_\delta(0))}{\nu_\epsilon(\RR^n \setminus B_\delta(0))} + 1}= 0.
  \end{align*}
\end{proof}

Next define \emph{regularized weighted Riesz kernel}
\begin{align}\label{eqn:reg_weighted_riesz_kernel}
  k_{\epsilon}^p(\epsilon)(x,y) \defeq k_\epsilon(x, y) (p(x)p(y))^{-s/2n},
\end{align}
and similarly its normalized version
\begin{align}\label{eqn:normalized_reg_weighted_riesz_kernel}
  \hat{k}_{\epsilon}^p(\epsilon)(x,y) \defeq \hat{k}_\epsilon(x, y) (p(x)p(y))^{-s/2n},
\end{align}
Then $k_{\epsilon}^p$ and $\hat{k}_\epsilon^p$ are positive semidefinite kernels. 
Note that they may not have finite integrals since $p$ can decay faster than $k_\epsilon$.

Define the \emph{continuous energy functional} for a probability measure $\mu$ with respect to a kernel $k$ as
\begin{align}
\begin{split}\label{eqn:energy_functional}
  \mathcal{E}_k(\mu) &\defeq \frac{1}{2}\iint k(x, y) \dd \mu(x) \dd \mu(y).
\end{split}
\end{align}

Then the \emph{continuous regularized Riesz energy} is defined as
\begin{align}
\begin{split}\label{eqn:reg_riesz_energy_cont}
  \mathcal{E}_{k_\epsilon^p}(\mu) &\defeq \frac{1}{2}\iint k_{\epsilon}^p(x, y) \dd \mu(x) \dd \mu(y) 
  = \frac{1}{2}\iint k_\epsilon(x, y) (p(x)p(y))^{-s/2n}\dd \mu(x) \dd \mu(y).
\end{split}
\end{align}
Similarly we can defined the normalized version of the continuous regularized Riesz energy $\mathcal{E}_{\hat{k}_\epsilon^p}$.
These energy are not always finite.


\subsection{Limiting energy as $\chi^2$-divergence}

Let $\mu^*_\alpha$ be the probability distribution so that its density satisfies 
\begin{equation}
  p_{\mu^*_\alpha}(x) \propto p(x)^\alpha.
\end{equation}

We show that limiting energy $\mathcal{E}_{\hat{k}_\epsilon^p}(\mu)$ can be intrepreted as the $\chi^2$-divergence between $\mu$ and $\mu^*_{s/n}$.
\begin{proposition}\label{prop:lim_chi_square}
  \lingxiao{Fix normalization.}
  Suppose $\mu$ is a probability measure with density $q(x)$. Then
  \begin{align*}
    \lim_{\epsilon \to 0} \mathcal{E}_{\hat{k}_\epsilon^p}(\mu) = \chi^2 \infdivx{\mu}{\mu^*_{s/n}} + 1,
  \end{align*}
  where
  \begin{align}\label{eqn:chi_square_divergence}
    \chi^2 \infdivx{Q}{P} \defeq \int \left(\frac{\dd Q}{\dd P} - 1\right)^2 \dd P.
  \end{align}

  In particular, 
  \begin{align*}
    \lim_{\epsilon \to 0} \mathcal{E}_{\hat{k}_\epsilon^p}(\mu^*_{s/n}) = 1.
  \end{align*}
\end{proposition}
\begin{proof}
  We compute using Tonelli's theorem (since our integrand is positive):
  \begin{align*}
    \mathcal{E}_{\hat{k}_\epsilon^p}(\mu) &= \iint \hat{k}_\epsilon(x, y) (p(x)p(y))^{-s/2n} \dd \mu(x) \dd\mu(y) \\
                                          &= \iint \hat{k}_\epsilon(x, y) (p(x)p(y))^{-s/2n} q(x) q(y) \dd x \dd y \\
                                          &= \int \EE_{Z \sim \nu_\epsilon}[p(x+Z)^{-s/2n} q(x+Z)] p(x)^{-s/2n} \dd \mu(x),
  \end{align*}
  where $\nu_\epsilon$ is defined in \eqref{eqn:reg_riesz_kernel}
  Then since $\nu_\epsilon$ converges in probability (hence in distribution) to $\delta_0$ by \cref{prop:kernel_measure_conv_delta}, we have \lingxiao{justify exchanging limit and integration, and continuity}
  \begin{align*}
    \lim_{\epsilon \to 0} \mathcal{E}_{\hat{k}_\epsilon^p}(\mu) &= \lim_{\epsilon \to 0}\int \EE_{Z \sim \nu_\epsilon} [p(x+Z)^{-s/2n} q(x+Z)] p(x)^{-s/2n} \dd \mu(x) \\
                                                                &= \int \lim_{\epsilon \to 0}\EE_{Z \sim \nu_\epsilon} [p(x+Z)^{-s/2n} q(x+Z)] p(x)^{-s/2n} \dd \mu(x) \\
                                                                &= \int [p(x)^{-s/2n} q(x)] p(x)^{-s/2n} \dd \mu(x) \\
                                                                &= \int \frac{q(x)^2}{p(x)^{s/n}} \dd x = \int \left(\frac{q(x)}{p(x)^{s/n}}\right)^2 \dd\mu^*_{s/n}(x) 
                                                                = \int \left(\frac{\dd\mu}{\dd\mu_{s/n}^*}(x)\right)^2 \dd\mu^*_{s/n}(x) \\
                                                                &= \int \left(\frac{\dd\mu}{\dd\mu_{s/n}^*}(x) - 1\right)^2 \dd\mu^*_{s/n}(x) + 1 = \chi^2\infdivx{\mu}{\mu^*_{s/n}} + 1.
  \end{align*}
\end{proof}
Note that we cannot use $\chi^2$-divergence defined in \eqref{eqn:chi_square_divergence} directly for particle-based sampling since it requires the evolving measure to have density. 
Our regularization \eqref{eqn:reg_riesz_energy_cont} can thus be viewed as a way to bypass such an obstacle.

\subsection{Stationary measure in Wasserstein space}
In this section our goal is to establish non-asymptotic bounds in terms of $\epsilon$ of the Wasserstein gradients of our energy \eqref{eqn:reg_riesz_energy_cont}.
Recall the following facts about Wasserstein gradients. \lingxiao{cite Ambrosio.}
\begin{proposition}\label{prop:W_2_gf_facts}
  Let $\mathcal{F}: \mathcal{P}_2(\RR^n) \to (-\infty, \infty]$ be a functional given by
  \[
    \mathcal{F}(\mu) = \int B(x) \dd \mu(x) + \iint \frac{1}{2} C(x) \dd \mu(x) \dd \mu(y)
  .\]
  \lingxiao{Regularity conditions on $B, C$?}
  Then the first variation of $\mathcal{F}$ is given by, $\mathcal{F}'(\mu): \RR^n \to \RR$, as
  \begin{align}
    \mathcal{F}'(\mu)(x) &= B(x) + \int C(x, y) \dd\mu(y).
  \end{align}
  The Wasserstein-2 gradient $\nabla_{W_2}\mathcal{F}(\mu): \RR^n \to \RR^n$ is given by
  \begin{align}
    \nabla_{W_2} \mathcal{F}(\mu)(x) &= \nabla_x \mathcal{F}'(\mu)(x) =  \nabla B(x) + \nabla \left(\int C(x, y) \dd \mu(y)\right).
  \end{align}
\end{proposition}

In the following analysis, we will show that for $s > n$, the probability measure $\mu^*_{s/n}$ is stationary with respect to $\mathcal{E}_{\hat{k}_\epsilon^p}$ as $\epsilon \to 0$.

\begin{proposition}\label{prop:conv_grad_vanish}
  \lingxiao{TODO: simplify the result in the main text assuming $\grad \log p$ is Lipschitz.}
  Suppose there exists $b \ge 1, M > 0$  and a function $K: \RR^n \to \RR_{> 0}$ such that $s > n + b$ and for every $x$, with $\norm{h}_2 \ge 1$, $p(x) > 0$, $p(x) < M$, $\log p(x)$ is continuous differentiable and satisfies
  \begin{align}\label{eqn:grad_log_p_poly_bound}
    \forall h\in \RR^n \setminus B_1(0), \quad \norm{\nabla \log p(x+h) - \nabla \log p(x)}_2 \le K(x) \norm{h}_2^b,
  \end{align}
  i.e., the growth of $h \mapsto \norm{\nabla \log p(x + h) - \nabla \log p(x)}_2$ is at most polynomial of degree $b$ outside of the unit ball.
  Then for every $x$ and $\epsilon \in (0, 1)$, we have 
  \begin{align}
    &\norm{\nabla_{W_2}\mathcal{E}_{k_\epsilon^p}(\mu^*_{s/n})(x)}_2 \le M(x) C \epsilon^{n+1-s},\label{eqn:unnormalized_bound} \\
    &\norm{\nabla_{W_2}\mathcal{E}_{\hat{k}_\epsilon^p}(\mu^*_{s/n})(x)}_2 \le M(x) C' \epsilon.\label{eqn:normalized_bound}
  \end{align}
  where $M(x)$ is a function that only depends on $x$, and $C, C'$ are constants depending only on $s, n, b$.
  Therefore, $\lim_{\epsilon \to 0}\norm{\nabla_{W_2}\mathcal{E}_{\hat{k}_\epsilon^p}(\mu^*_{s/n})(x)}_2 = 0$.
\end{proposition}
\begin{proof}
  With a slight abuse of notation, we write $k_\epsilon(x-y) = k_\epsilon(x, y)$.
  We compute \lingxiao{there is an unjustified interchange of integration and differentiation.}
  \begin{align*}
    &\quad\norm{\nabla_{W_2}\mathcal{E}_{k_\epsilon^p}(\mu^*_{s/n})(x)}_2 
    =\norm{\nabla_x \int k_{\epsilon, p}(x, y) \dd\mu^*_{s/n}(y)}_2 \\
    =&\norm{\nabla_x \int k_\epsilon(x - y)p(x)^{-s/2n} p(y)^{-s/2n} \dd\mu^*_{s/n}(y)}_2 \\
    =&\norm{\nabla_x \left(p(x)^{-s/2n} \int k_\epsilon(x - y)p(y)^{s/2n} \dd y\right)}_2 \\
    =&\norm{\nabla_x \left(p(x)^{-s/2n} \int k_\epsilon(y)p(x-y)^{s/2n} \dd y\right)}_2 \\
    =&\norm{\int k_\epsilon(y) \nabla_x \left( (p(x-y)/p(x))^{s/2n} \right)\dd y}_2 \\
    =&\norm{\int k_\epsilon(y) \nabla_x e^{\frac{s}{2n}(\log p(x-y) - \log p(x))} \dd y}_2 \\
    =&\norm{\int k_\epsilon(y)  e^{\frac{s}{2n}(\log p(x-y) - \log p(x))}(\nabla \log p(x-y) -\nabla \log p(x)) \dd y}_2 \\
    \le&  \int k_\epsilon(y)  e^{\frac{s}{2n}(\log p(x-y) - \log p(x))}\norm{\nabla \log p(x-y) -\nabla \log p(x)}_2 \dd y.
  \end{align*}
  Taking out the exponential factor using $p(x) < M$ and applying \eqref{eqn:grad_log_p_poly_bound}, we have
  \begin{align*}
    \norm{\nabla_{W_2}\mathcal{E}(\mu^*_{s/n})(x)}_2 
    \le  M^{s/2n} p(x)^{-s/2n} K(x) \int k_\epsilon(y) \norm{\nabla \log p(x-y) -\nabla \log p(x)}_2 \dd y.
  \end{align*}
  By Taylor's theorem, continuous differentiability of $\log p$ and the compactness of $B_1(0)$ imply that there exists $L(x)$ such that
  \begin{align*}
    \forall h \in B_1(0),\quad \norm{\nabla \log p(x+h) - \nabla \log p(x)}_2 \le L(x) \norm{h}_2.
  \end{align*}
  Combining this with \eqref{eqn:grad_log_p_poly_bound}, we have
  \begin{align*}
    \norm{\nabla \log p(x+h) - \nabla \log p(x)}_2 \le (L(x) + K(x)) (\norm{h}_2 + \norm{h}^b_2).
  \end{align*}
  Thus
  \begin{align*}
    \norm{\nabla_{W_2}\mathcal{E}(\mu^*_{s/n})(x)}_2  \le&  M^{s/2n} p(x)^{-s/2n} (L(x)+K(x)) \int k_\epsilon(y) (\norm{y}_2 + \norm{y}_2^b) \dd y \\
    =& M^{s/2n} p(x)^{-s/2n} (L(x)+K(x)) \left(\int (\norm{y}^2_2+\epsilon^2)^{-s/2} (\norm{y}_2 + \norm{y}_2^b) \dd y \right).
  \end{align*}

  To bound the last integral, since $s > n + b$, by \eqref{eqn:kernel_int_eq} and \eqref{eqn:kernel_int_complement_ub} with $\delta = \epsilon$, 
  \begin{align*}
    \int (\norm{y}^2_2+\epsilon^2)^{-s/2} \norm{y}_2^b \dd y &\le \mathcal{H}_{n-1}(S^{n-1}) \epsilon^{n+b-s} \left( \int_0^1 \frac{t^{n+b - 1}}{(t^2+1)^{s/2}}\dd t + \frac{1}{s-(n+b)} \right). 
  \end{align*}
  Similarly since $s > n + 1$,
  \begin{align*}
    \int (\norm{y}^2_2+\epsilon^2)^{-s/2} \norm{y}_2 \dd y &\le \mathcal{H}_{n-1}(S^{n-1}) \epsilon^{n+1-s} \left( \int_0^1 \frac{t^{n}}{(t^2+1)^{s/2}}\dd t + \frac{1}{s-(n+1)} \right). 
  \end{align*}
  Combining everything together we have
  \begin{align*}
    \norm{\nabla_{W_2}\mathcal{E}(\mu^*_{s/n})(x)}_2 
    \le M^{s/2n} \mathcal{H}_{n-1}(S^{n-1}) p(x)^{-s/2n}(L(x)+K(x))\left( A\epsilon^{n+b-s} + B \epsilon^{n+1-s} \right),
  \end{align*}
  where
  \begin{align*}
    A &= \int_0^1 \frac{t^{n+b - 1}}{(t^2+1)^{s/2}}\dd t + \frac{1}{s-(n+b)}, \qquad
    B = \int_0^1 \frac{t^{n}}{(t^2+1)^{s/2}} \dd t + \frac{1}{s-(n+1)}.
  \end{align*}
  Since $\epsilon < 1$, this proves \eqref{eqn:unnormalized_bound}.

  To obtain \eqref{eqn:normalized_bound}, simply observe that by \eqref{eqn:kernel_int_eq},
  \begin{align*}
    I_\epsilon &= \int k_\epsilon(0, x) \dd x = \int (\norm{y}_2^2+\epsilon^2)^{-s/2}\dd y 
    \ge \int_{B_\epsilon(0)} (\norm{y}_2^2+\epsilon^2)^{-s/2}\dd y \\
               &= \mathcal{H}_{n-1}(S^{n-1})\left(\int_0^1 \frac{t^{n-1}}{(t^2+1)^{s/2}}\dd t\right)\epsilon^{n-s}.
  \end{align*}
  Hence using \eqref{eqn:unnormalized_bound}, we have
  \begin{align*}
    \norm{\nabla_{W_2}\mathcal{E}_{\hat{k}_\epsilon^p}(\mu^*_{s/n})(x)}_2 &= \frac{\norm{\nabla_{W_2}\mathcal{E}_{k_\epsilon^p}(\mu^*_{s/n})(x)}_2}{I_\epsilon} 
    \le M(x) C' \epsilon.
  \end{align*}
\end{proof}

In our algorithm, we use the logarithmic Riesz energy for numerical stability.
We next show that $\mu^*_{s/n}$ is also a stationary measure for $\log \mathcal{E}_{k_\epsilon^p}$ as $\epsilon \to 0$.

\begin{corollary}
  Under the assumptions of \cref{prop:conv_grad_vanish}, we have
  \begin{align*}
    \norm{\nabla_{W_2} \log \mathcal{E}_{k_\epsilon^p}(\mu^*_{s/n})(x)}_2 &\le \frac{M(x)C \epsilon^{\min(b,1)}}{\mathcal{E}_{k_\epsilon^p}(\mu^*_{s/n})}.
  \end{align*}
  In particular, as $\epsilon \to 0$, $\mu^*_{s/n}$ is a stationary measure of the logarithm of \eqref{eqn:reg_riesz_energy_cont}, i.e.,
  \begin{align}
    \lim_{\epsilon \to 0}\norm{\nabla_{W_2} \log \mathcal{E}_{k_\epsilon^p}(\mu^*_{s/n})(x)}_2 = 0.
  \end{align}
\end{corollary}
\begin{proof}
  Note that the Wasserstein gradient of the logarithm of a functional is invariant to scaling. Hence,
  \begin{align*}
    \nabla_{W_2} \log \mathcal{E}_{k_\epsilon^p}(\mu^*_{s/n})(x) = \nabla_{W_2} \log \mathcal{E}_{\hat{k}_\epsilon^p}(\mu^*_{s/n})(x) = \frac{\nabla_{W_2}\mathcal{E}_{\hat{k}^p_\epsilon}(\mu^*_{s/n})(x)}{\mathcal{E}_{\hat{k}_\epsilon^p}(\mu^*_{s/n})}.
  \end{align*}
  Then the result is a simple consequence of \cref{prop:conv_grad_vanish} and \cref{prop:lim_chi_square}.
\end{proof}

\subsection{Connection to MMD}
The previous calculation also reveals a close connection with MMD with kernel $\hat{k}_{\epsilon}^p(x,y)$ defined in \eqref{eqn:reg_weighted_riesz_kernel}.
\begin{proposition}
Assume the same assumptions as in \cref{prop:conv_grad_vanish}.
As $\epsilon \to 0$, the gradient flow of $\frac{1}{2}\MMD^2_{\hat{k}_{\epsilon}^p}(\cdot,\mu^*_{s/n})$ and that of $\mathcal{E}_{\hat{k}_{\epsilon}^p}$ coincide, i.e., for any $x$,
  \begin{align*}
  \lim_{\epsilon \to 0} \norm{\nabla_{W_2} \left(\frac{1}{2}\MMD^2_{\hat{k}_{\epsilon}^p}(\mu, \mu^*_{s/n})\right)(x) - \nabla_{W_2}\mathcal{E}_{\hat{k}_{\epsilon}^p}(\mu)(x)}_2 = 0.
  \end{align*}
\end{proposition}
\begin{proof}
By definition,
\begin{align*}
\MMD^2_{\hat{k}_{\epsilon}^p}(\mu, \mu^*_{s/n}) &= \iint \hat{k}_\epsilon^p(x,y) (\dd\mu(x) - \dd\mu^*_{s/n}(x))(\dd\mu(y) - \dd\mu^*_{s/n}(y)) \\
    &= \iint \hat{k}_\epsilon^p(x, y)(\dd\mu(x) - 2\dd\mu^*_{s/n}(x))\dd\mu(y)  + C,
\end{align*}
where $C$ is a constant depending only on $\mu^*_{s/n}$.
Comparing with \eqref{eqn:reg_riesz_energy_cont}, we see that 
\begin{align*}
    \frac{1}{2}\MMD^2_{\hat{k}_\epsilon^p}(\mu, \mu^*) - \mathcal{E}_{\hat{k}_{\epsilon}^p}(\mu) &= - \int \left( \int \hat{k}_\epsilon^p(x,y)\dd\mu^*_{s/n}(x) \right)\dd\mu(y) + C \\
    &= - \int \left( \int \hat{k}_\epsilon^p(x,y)\dd\mu^*_{s/n}(y) \right)\dd\mu(x) + C.
\end{align*}
Since by \cref{prop:W_2_gf_facts}, $\nabla_{W_2}(\int f \dd \mu)(x) = \nabla f(x)$, the Wasserstein-2 gradient of this functional is
\begin{align*}
  \nabla_{W_2}\left(\frac{1}{2}\MMD^2_{\hat{k}_\epsilon^p}(\mu, \mu^*) - \mathcal{E}_{\hat{k}_{\epsilon}^p}(\mu)\right)(x) &= -\nabla_x \left( \int \hat{k}_{\epsilon}^p(x,y)\dd\mu^*_{s/n}(y) \right) \\
&= -\nabla_{W_2}\mathcal{E}_{\hat{k}_{\epsilon}^p}(\mu^*_{s/n})(x).
\end{align*}
The conclusion of \cref{prop:conv_grad_vanish} then yields the desired result.
\end{proof}
Hence the gradient flow of $\mathcal{E}_{\hat{k}_{\epsilon}^p}$ is not that different from that of $\frac{1}{2}\MMD^2_{\hat{k}_\epsilon^p}(\cdot, \mu^*_{s/n})$, except we cannot directly use $\MMD$ for sampling because during optimization it requires sample access to $\mu^*_{s/n}$.
Therefore our method can be viewed as a modification of an MMD flow with kernel $\hat{k}_\epsilon^p$ for sampling. 
On the other hand, our method remains biased in the continuous case because $\epsilon > 0$ (but discretization of $\mu$ into particles will introduce biases anyway).

\subsection{Displacement convexity}
In this section we investigate at what conditions our objective \eqref{eqn:reg_riesz_energy_cont} is displacement convex.
We will use abbreviations $k \defeq \hat{k}_{\epsilon}^p$ and $\mathcal{E} \defeq \mathcal{E}_{\hat{k}_\epsilon^p}$, 

\begin{proposition}
Let $\mu \in \mathcal{P}_2(\RR^n)$ and let $\psi \in C_c^\infty(\RR^n)$. Consider the path $\rho_t \defeq (I + t\nabla\psi)_\# \mu$. Then
\begin{align}
\begin{split}
  \dv[2]{}{t} \mathcal{E}(\rho_t) &= \EE_{x,y\sim\mu}[\nabla\psi(x)^\top \nabla_2\nabla_1 k(x, y) \nabla\psi(y)] 
  + \EE_{x,y\sim\mu}[ \nabla\psi(x)^\top H_1k(x, y)\nabla\psi(x)] 
   ,\label{eqn:dis_hess}
\end{split}
\end{align}
where $H_1 k$ is the Hessian of $k$ with respect to the first component and $\nabla_i k$ is the gradient with respect to the $i$th component.
\end{proposition}
\begin{proof}
The computation is similar to that in Proposition 3 of \citet{korba2021kernel}.
\end{proof}
Geodesic convexity of the functional $\mathcal{E}$ means $\dv[2]{}{t} \mathcal{E}(\rho_t) \ge 0$.
For the second term in \eqref{eqn:dis_hess}, we compute using the reproducibility of the the RKHS $\mathcal{H}$ associated with kernel $k$,
\begin{align*}
     &\EE_{x,y\sim\mu}[\nabla\psi(x)^\top \nabla_2\nabla_1 k(x, y) \nabla\psi(y)]\\
  =& \EE_{x,y\sim\mu} \left[ \langle \nabla\psi^\top(x)\nabla_1 k(x,\cdot), \nabla\psi^\top(y)\nabla_1 k(y,\cdot) \rangle \right] \\
     =& \norm{\EE_{x\sim\mu}[\nabla\psi^\top(x)\nabla_1 k(x,\cdot)] }_{\mathcal{H}}^2 \ge 0.
\end{align*}

For the first term, note that
\begin{align*}
  &\EE_{x,y\sim \mu}[ \nabla\psi(x)^\top H_1k(x, y)\nabla\psi(x)] \\
  =& \EE_{x\sim \mu}[ \nabla\psi(x)^\top H_1 (\EE_{y\sim \mu}[k(x, y)])\nabla\psi(x)] \\
  =& \EE_{x\sim \mu}[ \nabla\psi(x)^\top H_1 (\EE_{y\sim \mu}[k_\epsilon(x, y)(p(x)p(y))^{-s/2n}])\nabla\psi(x)].
\end{align*}
Hence this term will be nonnegative if $x \mapsto \EE_{y\sim \mu}[k_\epsilon(x, y)(p(x)p(y))^{-s/2n}]$ is a convex function.

Suppose $\mu$ has density $q(x)$. Then
\begin{align*}
  \EE_{y\sim \mu}[k_\epsilon(x, y)(p(x)p(y))^{-s/2n}] &= \int k_\epsilon(x,y)(p(x)p(y))^{-s/2n} q(y) \dd y \\
                                                      &= \EE_{Z\sim\nu_\epsilon} \left[\frac{q(x+Z)}{p(x)^{s/2n}p(x+Z)^{s/2n}}\right], \numberthis\label{eqn:dis_conv_need_cvx}
\end{align*}
where $\nu_\epsilon$ is defined in \eqref{eqn:riesz_kernel_measure}.
If $q \propto p^{s/n}$ (i.e. $\mu = \mu^*_{s/n}$), then the last term becomes
\begin{align*}
  \EE_{Z\sim\nu_\epsilon} \left[p(x)^{-s/2n}p(x+Z)^{s/2n}\right],
\end{align*}
which goes to $1$ as $\epsilon \to 0$.
So in particular it is convex.
On the other hand, if $p(x)$ is strongly log-concave, then the convexity could still hold at $\mu \neq \mu^*_{s/n}$.
\lingxiao{Find more general conditions for $\mu$ and $p$ under which \eqref{eqn:dis_conv_need_cvx} is convex for $\mu$ and make this section more formal.}





==> app_hessian_chi_square.tex <==

\subsubsection{Hessian of chi-square divergence}%


\begin{proposition}\label{prop:hessian_chi_square}
Assume that $\mu^*$ has a density $p(x)\propto \exp(-V(x))$ for some potential $V:X \to \RR$. 
The Hessian of $\chi^2(\cdot|\mu^*)$ at $\mu$ is given, for any $\psi \in C_c^{\infty}(X)$, by: 
\begin{equation*}
 \Hess_{\mu}\chi^2(\psi,\psi) = \int \left(\frac{q(x)}{p(x)} \right)^2 \left[\left(\mathcal{L}_{p}\psi(x)\right)^2 + \ps{\hess_V(x)\nabla \psi(x), \nabla \psi(x)} + \| \hess \psi(x)\|^2_{HS} \right] p(x)\dd x,
\end{equation*}
where $\hess_V$ is the Hessian of $V$, and $\mathcal{L}_p:\psi \mapsto \ps{\nabla V,\nabla \psi} - \Delta \psi$ is the Langevin diffusion operator associated to $p$ \citet[Section 4.5]{pavliotis2014stochastic}. 
In particular, if $V$ is convex, then $\chi^2(\cdot|\mu^*)$ is displacement convex.
\end{proposition}


To ensure fast decay of the Wasserstein gradient flow of the chi square divergence, we actually need strong (displacement) convexity, which can be obtained by lower bounding the Hessian by a quadratic form on the tangent space of the Wasserstein space, i.e. $\Hess_{\mu} \chi^2(\psi,\psi)\ge \lambda \|\nabla \psi\|^2_{L^2(\mu)}$ for any $\psi \in C_c^{\infty}(X)$. The latter holds if $\mu^*$ satisfies a Poincaré inequality and $V$ is convex \cite{chewi2020svgd}\ak{check/explain more the previous statement}.

Displacement convexity of the objective functional is fundamental since it is required for the global convergence of the Wasserstein gradient flow, hence a nice convergence behavior of any algorithm based on its time discretization. While the interaction energy $\mathcal{E}_{\epsilon}$ is not displacement convex in general even for a log-concave target, its gradient flow can be easily computed; in contrast $\chi^2(\cdot|\mu^*)$ is displacement convex but its gradient flow is not implementable. Hence, approximating the gradient flow of the chi-square divergence by the mollified Riesz energy realizes an interesting tradeoff between attractive geometric properties for optimization (displacement convexity) and computational tractability. 

\begin{proof}
Let $\mu_t = (\Id +t\nabla \psi)_{\#}\mu$ where $\psi \in C_c^{\infty}(\RR^n)$.
Let $q_t,q$ the densities of $\mu_t, \mu$ respectively.
 We denote by $\phi_t = \Id+ t g$ where $g= \nabla \psi$.
Hence we have $\J \phi_t = \Id +t \J g$. 
Time derivatives are denoted as $\phi'_t =\frac{d \phi_t}{d t}$. Notice that $(\J \phi_t)' = \J \phi'_t = \J g = \Hess \psi$.

For any $f$-divergence, 
  \begin{equation*}
      h_{\mu}(t) = \int f\left( \frac{q_t(x)}{p(x)}\right) p(x)\dd x = \int  \tf\left( \frac{q_t(x)}{p(x)}\right) q_t(x) \dd x.
  \end{equation*}
  where $\tilde{f}(t)=f(t)/t$. By the transfer lemma and change of variables formula\ak{justify diffeomorphism}, we have
  \begin{equation*}
       h_{\mu}(t) =  \int \tf \left(\frac{q(x) }{p( \phi_t(x))|\J \phi_t(x)|} \right) \dd q(x). 
  \end{equation*}
  Let us rewrite 
\begin{equation*}
    h_{\mu}(t) =  \int \tf \left(q(x) e^{n_t(x)} \right) \dd q(x), \quad \text{ where }\quad n_t(x)= V(\phi_t(x)) - \log |\J \phi_t(x)|.
\end{equation*}
We have consecutively\ak{justify deriving wrt to time in the integral}: 
\begin{align*}
    h'_{\mu}(t) &= \int \tf' \left(q(x)  e^{n_t(x)} \right) q(x) n'_t(x) e^{n_t(x)}\dd q(x)\\
    h''_{\mu}(t)&= \int \left[ \tf''( q(x) e^{n_t(x)}) \left(q(x)n'_t(x)e^{n_t(x)}\right)^2\right.\\
    & \left. \tf'( q(x) e^{n_t(x)})  \left( n''_t(x)+ n'_t(x)^2 \right)q(x) e^{n_t(x)} \right]q(x)dx
\end{align*}
where
\begin{align*}
   n'_t(x) &= \ps{\nabla V(\phi_t(x)), \phi'_t(x)} - \Tr \left( (\J \phi_t(x))^{-1} \J \phi'_t(x) \right),  \\
   n''_t(x)&= \ps{\hess_V (\phi_t(x)) \phi'_t(x), \phi'_t(x)} + \Tr \left( \left( \J \phi_t(x))^{-1} \J \phi'_t(x)\right)^2 \right),
\end{align*}
since $\phi''_t = 0$. 
At time $t=0$, we have 
\begin{align*}
n_0(x)&= V(x) = - \log(p(x))\\
    n'_0(x)&= \ps{\nabla V(x), \nabla \psi(x)} -\Delta \psi(x),\\
    n''_0(x)& = \ps{\hess_V(x)\nabla \psi(x), \nabla \psi(x)} + \| \hess \psi(x)\|^2_{HS}
\end{align*}
since  $\Tr \left( \hess \psi\right) = \Delta \Psi$ and $\Tr \left( (\hess \psi)^2\right) = \| \hess \psi\|^2_{HS}$.
Notice that $n'_0(x)=\mathcal{L}_{p}\psi (x)$ where $\mathcal{L}_{p}:\psi \mapsto  \ps{\nabla V, \nabla \psi} - \Delta \psi$ denotes the (negative) generator of the standard Langevin
diffusion with stationary distribution $\mu^*$ with density $p\propto e^{-V}$, see \citet[Section 4.5]{pavliotis2014stochastic}.

Now we get 
\begin{multline*}
    h''_{\mu}(0)= \int \left [\left( \tf'' \left(\frac{q(x)}{p(x)}\right) \left(\frac{q(x)}{p(x)} \right)^2 +  \tf'\left(\frac{q(x)}{p(x)}\right)  \left(\frac{q(x)}{p(x)}\right) \right) \left( \mathcal{L}_{p}\psi(x) \right)^2  \right.
    \\
    \left.+ \tf'\left(\frac{q(x)}{p(x)}\right)  \left(\frac{q(x)}{p(x)}\right)
   \left( \ps{\hess_V(x)\nabla \psi(x), \nabla \psi(x)} + \| \hess \psi(x)\|^2_{HS}\right)
    \right]q(x)dx.
\end{multline*}
Hence if $V$ is convex, and that $\min(\tf'(t), t\tf'(t)+ t^2\tf''(t)) \ge 0$, then $h''_{\mu}(0)\ge 0$.\ak{I think the formula is correct, at least I recover the formula for the KL -see  \cite{wibisono2018sampling} - the first term above in the formula is zero for f(t)=tlog t-t}

Now let $f(t)=t^2 - t$, then $h_{\mu}(t)=\chi^2(\mu_t|\mu^*)$. Moreover $\tf'(t)=1, \tf''(t)=0$ and we obtain the geodesic convexity of $\chi^2(\cdot|\mu^*)$ when $\mu^*$ is log-concave.  Moreover the Hessian of $\chi^2(\cdot|\mu^*)$ at $\mu$ can be written:
\begin{equation*}
    \Hess_{\mu}\chi^2(\psi,\psi) = \int \left(\frac{q(x)}{p(x)} \right)^2 \left[\left(\mathcal{L}_{p}\psi(x)\right)^2 + \ps{\hess_V(x)\nabla \psi(x), \nabla \psi(x)} + \| \hess \psi(x)\|^2_{HS} \right] p(x)\dd x.\qedhere
\end{equation*}
\end{proof}


\subsubsection{Tentative to prove convergence of Hessians \ak{not finished}}




For the interaction energy at $\mu=\mu^*$
\begin{multline}
    \Hess_{\mu} \mathcal{E}_{\eps}(\psi, \psi) =\iint\left[ \nabla \psi^\top(x)\nabla_1 \nabla_2 W_\eps(x,y)\nabla\psi(y)\right]\dd \mu(x)\dd \mu(y) \\+ \iint\left[ \nabla\psi^\top(x)\hess_1 W_\eps(x,y)\nabla\psi(x)\right]\dd \mu(x)\dd \mu(y)\\
    := \Hess_{p}\mathcal{F}_1(\psi,\psi) + \Hess_{p}\mathcal{F}_2(\psi,\psi).
\end{multline}
First notice that :
\begin{align*}
    \Hess_{\mu}\mathcal{F}_2(\psi,\psi)& = \int \nabla \psi(x)^T \hess_1 \left( \int W_{\epsilon}(x,y)\dd \mu(y)\right)\nabla \psi(x) \dd \mu(x)\\
    &\xrightarrow[\varepsilon \to 0]{}\int \nabla \psi(x)^T \hess_1 \left( \frac{q(x)}{p(x)}\right)\nabla \psi(x) \dd \mu(x) = 0 \text{ if } \mu=\mu^*.
\end{align*}
\ak{justify hessian/limit inversion}


By an integration by parts\footnote{First, differentiate the product $\frac{\partial \psi(x)}{\partial x_i}p(x)$, then integrate $\frac{\partial^2 W_{\epsilon}(x,y)}{\partial x_i \partial y_j}$ w.r.t.\ $x_i$. Since $\psi$ is compactly supported, it vanishes at infinity. Since $p$ has a $C^1$-density w.r.t.\ the Lebesgue measure, any integral over $\d p$ bearing on the boundary of the support of $p$ vanishes. We thus do not have any extra integral on the boundary when performing the integration by parts.} w.r.t.\ $x$, we have, for $\cL_{p} : f\mapsto-\Delta f+\langle - \nabla \log p,\nabla f \rangle$,
\begin{align*}%
\Hess_{p}\mathcal{F}_1&(\psi,\psi)
= \sum_{i,j=1}^d \iint \frac{\partial \psi(x)}{\partial x_i}. \frac{\partial^2 W_{\epsilon}(x,y)}{\partial x_i \partial y_j}. \frac{\partial \psi(y)}{\partial y_j}\dd p(x)\dd p(y)\\
&= - \sum_{i,j=1}^d \iint \frac{\partial^2 \psi(x)}{\partial x_i^2}. \frac{\partial W_{\epsilon}(x,y)}{\partial y_j}. \frac{\partial \psi(y)}{\partial y_j}\dd p(x)\dd p(y)\\
&- \sum_{i,j=1}^d \iint \frac{\partial \psi (x)}{\partial x_i}. \frac{\partial \log p(x)}{\partial x_i}. \frac{\partial W_{\epsilon}(x,y)}{\partial y_j}. \frac{\partial \psi(y)}{\partial y_j}\dd p(x)\dd p(y)\\
&= \sum_{j=1}^d\iint \cL_p\psi(x).\frac{\partial W_{\epsilon}(x,y)}{\partial y_j}. \frac{\partial \psi(y)}{\partial y_j}\dd p(x)\dd p(y).
\end{align*}
We then repeat the same steps, performing an integration by parts w.r.t.\ $y_j$ 
\begin{equation*}
   \Hess_{p}\mathcal{F}_1(\psi,\psi) = \int \cL_{p}\psi(x)W_{\epsilon}(x,y)\cL_{p}\psi(y)\dd p(x)\dd p(y)
\xrightarrow[\varepsilon \to 0]{} \int \left(\cL_{p}\psi(x) \right) ^2 \dd p(x).
\end{equation*}



For the chi square at $\mu=\mu^*$.
\begin{align*}
    \Hess_{\mu}\chi^2(\psi,\psi) = \int  \left[\left(\mathcal{L}_{p}\psi(x)\right)^2 + \ps{\hess_V(x)\nabla \psi(x), \nabla \psi(x)} + \| \Hess \psi(x)\|^2_{HS} \right] p(x)\dd x.\qedhere
\end{align*}
\ak{I think the formula of chi square can be simplified. below some trials commented.}
\ak{try an ipp on the last two terms}

\begin{equation*}
   \left(\mathcal{L}_{p}\psi(x)\right)^2= (\Delta \psi(x))^2 - 2\Delta \psi(x) \ps{\nabla \psi(x), \nabla V(x)} + \ps{\nabla \psi(x), \nabla V(x)}^2\end{equation*}

\ak{ with Bochner's formula see end of paper here \url{https://arxiv.org/pdf/2102.04413.pdf}}

We have by i.p.p\begin{multline*}    \int - 2\Delta \psi(x) \ps{\nabla \psi(x), \nabla V(x)}\dd p(x) =    \int 2\Delta \psi(x) \ps{\nabla \psi(x), \nabla p(x)}\dd x \\   =-2    \int \div \left( \nabla \psi(x)\Delta \psi(x) \right)p(x)\dd x\\    = - 2 \int \left[  \langle \div \Delta \psi(x),\nabla \psi(x)\rangle + (\Delta \psi(x))^2 \right] p(x)\dd x\end{multline*}And Bochner's formula yields:\begin{equation*}    \Delta \|\nabla \psi(x)\|^2 - 2  \langle \div \Delta \psi(x),\nabla \psi(x)\rangle =  2 \| \Hess \psi(x)\|^2.\end{equation*}Then we have, since $\psi$ is compactly supported \ak{see \url{https://mathoverflow.net/questions/187671/relationship-between-laplacian-and-hessian-on-compact-lie-groups}, can proved by an ipp apparently - to check but i think that's true only for $p$ uniform}:\begin{equation*}    \int \|\Hess \psi(x)\|^2 \dd p(x) = \int (\Delta \psi(x))^2 \dd p(x)\end{equation*}







==> app_mmd.tex <==
\subsection{Connection to MMD}
When $X$ is compact, \cref{prop:energy_cvx_signed} shows that $W_\eps$ defined in \eqref{eqn:weighted_kernel} is i.s.p.d.
This implies that the \emph{maximum mean discrepancy} $\MMD_{W_\eps}(\mu, \nu)$ defined by
\begin{align}
  \MMD^2_{W_\eps}(\mu, \nu) \defeq \iint W_\eps(x, y) (\dd \mu(x) - \dd \nu(x))(\dd \mu(y) - \dd \nu(y))
\end{align}
is a metric, i.e., the kernel $W_\eps$ is \emph{characteristic} \citep{sriperumbudur2010hilbert}, 
In particular, $\MMD_{W_\eps}(\mu, \nu) = 0$ if and only if $\mu = \nu$ (agree on all Borel sets).

Note that
\begin{align*}
  \MMD_{W_\eps}^2(\mu, \mu^*) = \mathcal{E}_\eps(\mu) - 2 \iint W_\eps(x, y) \dd\mu(x) \dd\mu^*(y) + C(\mu^*),
\end{align*}
where $C(\mu^*)$ depends only on $\mu^*$.
Define
\begin{align}
  \mathcal{G}_\eps(\mu) \defeq 2\iint W_\eps(x, y) \dd\mu(x) \dd\mu^*(y),
\end{align}
so that $\MMD_{W_\eps}^2(\mu, \mu^*) = \mathcal{E}_\eps(\mu) - \mathcal{G}_\eps(\mu) + C(\mu^*)$.
Observe that
\begin{align*}
  \mathcal{G}_\eps(\mu) &= 2 \iint \phi_\eps(x - y) (p(x)p(y))^{-1/2} p(y) \dd \mu(x) \dd y \\
                        &= 2 \int \left( \int \sqrt{p(y)}\phi_\eps(x - y) \dd y \right) p(x)^{-1/2} \dd\mu(x) \\
                        &= 2 \int \EE_{Y \sim \nu_\eps} \left[\sqrt{p(x- Y)}\right] p(x)^{-1/2} \dd\mu(x).
\end{align*}
For many choices of mollifiers, the distribution $\nu_\eps$ is in closed form and we can draw samples from it.
Hence $\mathcal{G}_\eps$ can be viewed as a debiasing term.
However, an issue is that the normalizing constant of $\tilde p(x)$ is unknown: in $\mathcal{E}_\eps(\mu)$ the normalizing constant shows up but in $\mathcal{G}_\eps(\mu)$ it does not.


==> app_proof_hessians.tex <==
\subsection{Proofs of \Cref{sec:geo_convexity}}



\subsubsection{Proof of \Cref{prop:hessian_interaction_energy}}



\begin{proof}
The function $f: t\mapsto W_{\epsilon}(x+t\nabla \psi(x),x'+t\nabla\psi(x'))$ is differentiable for all $x,x' \in X$, and its time derivative is :
\begin{align*}
        \dot{f}&=
        \nabla_{1} W_{\epsilon}(x+t\nabla\psi(x),x'+t\nabla\psi(x'))^{\top}\nabla\psi(x)
        + \nabla_{2} W_{\epsilon}(x+t\nabla\psi(x),x'+t\nabla\psi(x'))^{\top}\nabla\psi(x')\nonumber\\
            &=\nabla_{1} W_{\epsilon}(x+t\nabla\psi(x),x'+t\nabla\psi(x'))^{\top}\nabla\psi(x) + \nabla_{1} W_{\epsilon}(x'+t\nabla\psi(x'),x+t\nabla\psi(x))^{\top}\nabla\psi(x')
\end{align*}
using the symmetry of $W_{\epsilon}$ (for any $x,y\in X$, $\nabla_1 W_{\epsilon}(x,y)= \nabla_{2}W_{\epsilon}(y,x)$).
The two terms on the r.h.s. of the former equation are symmetric w.r.t.\ $x$ and $x'$, so we will focus on the first one.
By the Cauchy-Schwartz inequality 
\begin{align*}
|\nabla_1 W_{\epsilon}(x&+t\nabla \psi(x), x'+t\nabla\psi(x'))^{\top}\nabla \psi(x) |\leq \|\nabla_1 W_{\epsilon}(x+t\nabla \psi(x), x'+t\nabla\psi(x'))\| \|\nabla \psi(x)\|
\end{align*}
The r.h.s. of the above inequality 
is integrable in $x$ because $(x,y)\mapsto \| \nabla_1 W_{\epsilon}(x,y)\|$ is integrable $\nabla \psi$ is compactly supported.
Therefore, by the differentiation lemma \citep[Theorem 6.28]{klenke2013probability}, $\mathcal{E}_{\epsilon}(\mu_t)$ is differentiable and  %
\begin{equation*}%
	\dot{\mathcal{E}_{\epsilon}}(\mu_t)=\mathbb{E}_{\substack{x\sim \mu \\x'\sim \mu}}\left[\dot{f} \right]  =\mathbb{E}_{\substack{x\sim \mu \\x'\sim \mu}}\left[ \nabla_{1} W_{\epsilon}(x+t\nabla\psi(x),x'+t\nabla\psi(x'))^{\top}\nabla \psi(x)\right].
	\end{equation*}
Now define the function $g:t\mapsto \nabla_{1} W_{\epsilon}(x+t\nabla\psi(x),x'+t\nabla \psi(x'))^{\top} \nabla\psi(x)$. Its time derivative writes as
\begin{align*}
    \dot{g}&=\nabla\psi(x)^\top \nabla_2\nabla_1 W_{\epsilon}(x+t\nabla\psi(x),x'+t\nabla\psi(x'))\nabla\psi(x')\\
&\quad	+\nabla \psi(x)^\top H_1 W_{\epsilon}(x+t\nabla\psi(x),x'+t\nabla\psi(x') ) \nabla\psi(x).
\end{align*}
The first term on the r.h.s. is integrable in $(x,x')$ because it is compactly supported and continuous.
We now deal with the second term:
\begin{align*}
    |\nabla\psi(x)^\top H_1 W_{\epsilon}(x+t\nabla\psi(x)&,x'+t\nabla\psi(x') ) \nabla\psi(x)|\\
   & \quad \le \|H_1 W_{\epsilon}(x+t\nabla\psi(x),x'+t\nabla\psi(x') )\|_{op}\| \nabla\psi(x)\|^2
    \end{align*}
The r.h.s. of the above inequality is integrable because $(x,y)\mapsto \| H_1 W_{\epsilon}(x,y)\|_{op}$ is integrable and $\nabla \psi$ is compactly supported.
\end{proof}

\subsubsection{Proof of \Cref{prop:hessian_interaction_energy_at_mu_star}}


\begin{proof}
According to \Cref{prop:hessian_interaction_energy}, we have:
\begin{multline}
    \Hess_{\mu^*} \mathcal{E}_{\eps}(\psi, \psi) =\iint\left[ \nabla \psi^\top(x)\nabla_1 \nabla_2 W_\eps(x,y)\nabla\psi(y)\right]\dd \mu^*(x)\dd \mu^*(y) \\+ \iint\left[ \nabla\psi^\top(x)\hess_1 W_\eps(x,y)\nabla\psi(x)\right]\dd \mu^*(x)\dd \mu^*(y)\\
    := \Hess_{\mu^*}\mathcal{F}_1(\psi,\psi) + \Hess_{\mu^*}\mathcal{F}_2(\psi,\psi).
\end{multline}
First notice that :
\begin{align*}
    \Hess_{\mu^*}\mathcal{F}_2(\psi,\psi)& = \int \nabla \psi(x)^T \hess_1 \left( \int W_{\epsilon}(x,y)\dd \mu^*(y)\right)\nabla \psi(x) \dd \mu^*(x)\\
    &\xrightarrow[\varepsilon \to 0]{}\int \nabla \psi(x)^T \hess_1 \left( \frac{q(x)}{p(x)}\right)\nabla \psi(x) \dd \mu(x) = 0 .
\end{align*}
\ak{justify hessian/limit inversion}


Then, by an integration by parts\footnote{First, differentiate the product $\frac{\partial \psi(x)}{\partial x_i}p(x)$, then integrate $\frac{\partial^2 W_{\epsilon}(x,y)}{\partial x_i \partial y_j}$ w.r.t.\ $x_i$. Since $\psi$ is compactly supported, it vanishes at infinity. Since $p$ has a $C^1$-density w.r.t.\ the Lebesgue measure, any integral over $\d p$ bearing on the boundary of the support of $p$ vanishes. We thus do not have any extra integral on the boundary when performing the integration by parts.} w.r.t.\ $x$, we have, for $\cL_{p} : f\mapsto-\Delta f+\langle - \nabla \log p,\nabla f \rangle$,
\begin{align*}%
\Hess_{\mu^*}\mathcal{F}_1&(\psi,\psi)
= \sum_{i,j=1}^d \iint \frac{\partial \psi(x)}{\partial x_i}. \frac{\partial^2 W_{\epsilon}(x,y)}{\partial x_i \partial y_j}. \frac{\partial \psi(y)}{\partial y_j}\dd p(x)\dd p(y)\\
&= - \sum_{i,j=1}^d \iint \frac{\partial^2 \psi(x)}{\partial x_i^2}. \frac{\partial W_{\epsilon}(x,y)}{\partial y_j}. \frac{\partial \psi(y)}{\partial y_j}\dd p(x)\dd p(y)\\
&- \sum_{i,j=1}^d \iint \frac{\partial \psi (x)}{\partial x_i}. \frac{\partial \log p(x)}{\partial x_i}. \frac{\partial W_{\epsilon}(x,y)}{\partial y_j}. \frac{\partial \psi(y)}{\partial y_j}\dd p(x)\dd p(y)\\
&= \sum_{j=1}^d\iint \cL_p\psi(x).\frac{\partial W_{\epsilon}(x,y)}{\partial y_j}. \frac{\partial \psi(y)}{\partial y_j}\dd p(x)\dd p(y).
\end{align*}
We then repeat the same steps, performing an integration by parts w.r.t.\ $y_j$ 
\begin{equation*}
   \Hess_{p}\mathcal{F}_1(\psi,\psi) = \int \cL_{p}\psi(x)W_{\epsilon}(x,y)\cL_{p}\psi(y)\dd p(x)\dd p(y)
\xrightarrow[\varepsilon \to 0]{} \int \left(\cL_{p}\psi(x) \right) ^2 \dd p(x).\qedhere
\end{equation*}

\end{proof}



==> app_wgf.tex <==
\subsection{Wasserstein gradient flow of $\cE_\eps$}
The goal of this section is to rigorously establish the existence and uniqueness of the Wasserstein gradient flow in $\cP_2(\RR^n)$ of the mollified interaction energy $\cE_\eps$ under additional assumptions \cref{ass:wgf} (in particular the target density $p$ is bounded from below in order to circumvent integrability issues).
We first recall the Wasserstein gradient flow framework from \citet{craig2022blob}.
We denote the domain of a functional $\cF: \cP_2(\RR^n) \to (-\infty,\infty]$ to be $D(\cF) \defeq \{\mu \in \cP_2(\RR^n): \cF(\mu) < \infty\}$.
\begin{definition}[transport plans, and Wasserstein distance]
  Let $\mu, \nu \in \cP(\RR^n)$.
  For a Borel measurable map $\bm T: \RR^n \to \RR^n$, we say $\bm T$ is a \emph{transport map} from $\mu$ to $\nu$ if $\nu(A) = \mu(\bm T^{-1}(A))$ for all Borel sets $A$, and we write $\nu = \bm T_\# \mu$.
  The set of \emph{transport plans} from $\mu$ to $\nu$ is
  \[
    \Gamma(\mu, \nu) \defeq \{\bm\gamma \in \cP(\RR^n\times\RR^n): \pi^1_\#\bm\gamma = \mu, \pi^2_\#\bm\gamma = \nu\}
  ,\]
  where $\pi^1,\pi^2: \RR^n\times\RR^n \to \RR^n$ are projections onto the first and the second copy of $\RR^n$, respectively.
  The \emph{Wasserstein distance} between $\mu, \nu \in \cP_2(\RR^n)$ is given by
  \begin{equation}\label{eqn:W_2}
    W_2(\mu, \nu) \defeq \min_{\bm\gamma \in \Gamma(\mu, \nu)} \left( \int \norm{x-y}_2^2 \dd\bm\gamma(x,y) \right)^{-1/2}
    .
  \end{equation}
  A plan $\bm\gamma$ is \emph{optimal} if it attains the minimum in \eqref{eqn:W_2} and we denote the set of all optimal plans from $\mu$ to $\nu$ by $\Gamma_o(\mu, \nu)$.
\end{definition}

\begin{definition}[geodesics in the Wasserstein metric]
  Given $\mu_0, \mu_1 \in \cP_2(\RR^n)$, the \emph{geodesics} connecting $\mu_0$ to $\mu_1$ are curves of the form
  \[
    \mu_t = ((1-t)\pi^1 + t \pi^2)_\# \bm\gamma, \quad t \in [0,1], \bm\gamma \in \Gamma_o(\mu_0, \mu_1)
  .\]
  More generally, given $\mu_1, \mu_2, \mu_3 \in \cP_2(\RR^n)$, a \emph{generalized geoesic} from $\mu_2$ to $\mu_3$ with base $\mu_1$ is given by
  \begin{align*}
    \mu_t^{2\to 3} = ((1-t)\pi^2 + t\pi^3)_\#\bm\gamma, \quad& t \in [0, 1], \bm\gamma \in \cP((\RR^n)^3) \\
                                                          &\text{such that } \pi^{1,2}_\#\bm\gamma \in \Gamma_o(\mu_1,\mu_2), \pi^{1,3}_\#\bm\gamma \in \Gamma_o(\mu_1, \mu_3)
  ,
  \end{align*}
  where $\pi^{i,j}: (\RR^n)^3 \to (\RR^n)^2$ denote the projection onto the $i$th and $j$th copies of $\RR^n$.
\end{definition}

\begin{definition}[displacement convexity]
  A functional $\cF: \cP_2(\RR^n) \to (-\infty, \infty]$ is \emph{$\lambda$-displacement convex along generalized geodesics} for $\lambda \in \RR$ if, for all $\mu_1,\mu_2,\mu_3 \in \cP_2(\RR^n)$, there exists a generalized geodesic $\bm\gamma$ from $\mu_2$ to $\mu_3$ with base $\mu_1$ such that for all $t \in [0, 1]$, 
  \begin{equation}
    \cF(\mu_t^{2\to 3}) \le (1-t) \cF(\mu_2) + t \cF(\mu_3) - t(1-t)\frac{\lambda}{2} W^2_{2,\bm\gamma}(\mu_2,\mu_3),
  \end{equation}
  where 
  \[
    W^2_{2,\bm\gamma}(\mu_2, \mu_3) \defeq \int \norm{y-z}_2^2\dd\bm\gamma(x,y,z)
  .\]
\end{definition}

\begin{definition}[absolutely continuous curves in $\cP_2(\RR^n)$]
  We say $\mu: [0, T] \to \cP(\RR^n)$ is \emph{absolutely continuous} on $[0, T]$ and write $\mu \in \AC_\loc^2((0, T); \cP_2(\RR^n))$ if there exists $f \in L_\loc^2((0, T))$ such that for all $s,t$ satisfying $0 < s \le t < T$,
  $
    W_2(\mu(t), \mu(s)) \le \int_s^t f(r) \dd r.
  .$
\end{definition}

\begin{definition}[subdifferential of $\lambda$-convex functional]
  Suppose $\cF: \cP_2(\RR^n) \to (-\infty,\infty]$ is proper, l.s.c., and $\lambda$-convex along generalized geodesics.
  Let $\mu \in D(\cF)$ and $\bm w: \RR^n \to \RR^n$ with $\bm w \in L^2(\mu;\RR^n)$.
  We say that $\bm w$ is a \emph{subdifferential} of $\cF$ at $\mu$ and write $\bm w \in \partial \cF(\mu)$, if for all $\nu \in \cP(\RR^n)$,
  \[
    \cF(\nu) - \cF(\mu) \ge \int \bm w(x)^\top (y-x)\dd\bm\gamma(x,y) + \frac{\lambda}{2}W_2^2(\mu, \nu), \text{ for all } \bm\gamma \in \Gamma_o(\mu, \nu)
  .\]
\end{definition}

\begin{definition}[local slope]
  Given $\cF: \cP_2(\RR^n) \to (-\infty,\infty]$, for any $\mu \in D(\cF)$, the \emph{local slope} is
  \[
    \abs{\partial \cF}(\mu) \defeq \limsup_{\nu \to \mu}\frac{(\cF(\mu) - \cF(\nu))_+}{W_2(\mu, \nu)}
  ,\]
  where $(s)_+ \defeq \max(s,0)$ and the convergence $\nu \to \mu$ is in $W_2$ metric.
\end{definition}

We will use the following proposition which defines a criterion for the uniqueness of the min-norm subdifferential:
\begin{proposition}[min-norm subdifferential; \citet{craig2022blob}, Proposition 2.11]
  \label{prop:min_norm_subdiff}
  Suppose $\cF: \cP_2(\RR^n) \to (-\infty,\infty]$ is proper, l.s.c., and $\lambda$-convex along generalized geodesics.
  Then for any $\mu \in D(\abs{\partial \cF})$, we have,
  \[
    \abs{\partial \cF}(\mu) \le \inf\{\norm{\bm \xi}_{L^2(\mu;\RR^n)}: \bm\xi \in \partial\cF(\mu)\}
  ,\]
  If equality holds and there exists $\bm w \in \partial \cF(\mu)$ that attains the infimum on the right-hand side, then such min-norm subdifferential is unique and we write $\bm w = \partial^\circ\cF$.
\end{proposition}

We can now define the Wasserstein gradient flow of a $\lambda$-convex functional.
\begin{definition}[gradient flow]
  Suppose $\cF: \cP_2(\RR^n) \to (-\infty, \infty)$ is proper, l.s.c., and $\lambda$-convex along generalized geodesics. A curve $\mu(t) \in \AC^2_{\loc}((0, \infty);\cP_2(\RR^n))$ is a \emph{Wasserstein gradient flow of $\cF$} if  $\mu(t)$ is a weak solution of the continuity equation (when tested against $C_c^\infty((0,\infty) \times \RR^n)$),
  $
    \partial_t \mu(t) + \nabla \cdot (v(t)\mu(t)) = 0
    ,$ with $v(t) = -\partial^\circ \cF(\mu(t))$ for $\mathcal{L}_1\text{-a.e. }t > 0.$
\end{definition}
The $\lambda$-displacement convexity of the functional, even if $\lambda < 0$, is enough to guarantee the existence and uniqueness of Wasserstein gradient flows.
\begin{theorem}[existence and uniqueness of the gradient flow; \citet{craig2022blob}, Theorem 2.13]
  \label{thm:wgf_exist_unique}
  Suppose $\cF: \cP_2(\RR^n) \to (-\infty, \infty]$ is proper, l.s.c., and $\lambda$-convex along generalized geodesics, and $\mu(0) \in \overline{D(\cF)}$. Then there exists a unique Wasserstein gradient flow $\mu(t)$ of $\cF$ with $\lim_{t \to 0^+} \mu(t) = \mu(0)$.
\end{theorem}


We now show that $\cE_\eps$ is $\lambda$-displacement convex so that its Wasserstein gradient flow exists and is unique.
We will assume a different set of assumptions in this section.
\begin{assumption}\label{ass:wgf}
  Suppose the target density $p \in C^2(\RR^n)$ satisfies $1/C_p \le p(x) \le C_p$, $\norm{\nabla p(x)}_2 \le C_p'$, $\norm{\hess p(x)}_2 \le C_p''$ for all $x \in \RR^n$, where we use $\norm{A}_2$ to indicate the matrix spectral norm (i.e. $\norm{A}_2 = \sigma_{\max}(A)$).
  Suppose our mollifier $\phi_\eps \in C^2(\RR^n)$ satisfies, in addition to \cref{defn:mollifiers}, $\phi_\eps \le C_\eps$, $\norm{\nabla \phi_\eps(x)}_2 \le C_\eps'$ and $\norm{\hess \phi_\eps(x)}_2 \le C''_\eps$. 
  Furthermore, the kernel $k_\eps(x,y) \defeq \phi_\eps(x-y)$ is i.s.p.d. on any compact set.
\end{assumption}
It can be readily checked that the assumptions in \cref{ass:wgf} on the mollifiers are satisfied by the $s$-Riesz, Gaussian, and Laplace families of mollifiers.
Since $p$ is now bounded below, the target measure $\dd\mu^*(x) = p(x)\dd\cL_n(x)$ is infinite, but \eqref{eqn:mollified_energy} and \eqref{eqn:limit_energy} are still well-defined.

\begin{lemma}\label{lem:wgf_energy_dt}
  Let $\mu_1,\mu_2,\mu_3 \in \cP_2(\RR^n)$ and $\bm\gamma \in \cP_2((\RR^n)^3)$ with $\pi^i_\# \bm\gamma = \mu_i$ for $i \in \{1,2,3\}$. Consider the curve $\mu_t \defeq ((1-t)\pi^2+ t\pi^3)_\#\bm \gamma$ for $t \in [0, 1]$.
  Then for each $\eps > 0$,
  \begin{align*}
    \dv{}{t}\bigg|_{t=0} \cE_\eps(\mu_t) \defeq 2 \iint \nabla_1W_\eps(y,y')^\top(z-y)\dd\mu_2(y')\dd\bm\gamma(x,y,z).
  \end{align*}
\end{lemma}
\begin{proof}
  We compute
  \begin{align*}
    \cE_\eps(\mu_t) = \iint W_\eps((1-t)y+tz, (1-t)y'+tz') \dd\bm\gamma(x,y,z)\dd\bm\gamma(x',y',z').
  \end{align*}
  Since by definition $W_\eps(x,x') = \phi_\eps(x-x')p^{-1/2}(x)p^{-1/2}(x')$, by \cref{ass:wgf}, we see that $\norm{\nabla_1 W_\eps}_2,\norm{\nabla_2 W_\eps}_2$ are bounded, where we use $\nabla_i W_\eps$ to denote the gradient of $W_\eps$ with respect to the $i$th input.
  Since $\bm\gamma$ is a probability measure, applying the differentiation lemma \citep[Theorem 6.28]{klenke2013probability}, and using the fact that $W_\eps(x,x') = W_\eps(x',x)$, we have our designed result.
\end{proof}

\begin{lemma}\label{lem:mix_diff_kernel_ispd}
  If a kernel $K: \RR^n \times \RR^n \to \RR^n$ is i.s.p.d. on all compact sets and is continuously differentiable in each variable with $\sup_{x,y} \abs{\partial_{x_i}\partial_{y_j} K(x,y)} < \infty$ for all $i,j\in [n]$, then for any finite signed measure $\mu$, we have
  \[
    \sum_{i,j\in [n]}\iint \partial_{x_i}\partial_{y_j} K(x,y)\dd\mu(x)\dd\mu(y) \ge 0
  ,\]
\end{lemma}
\begin{proof}
  We first show the statement when $\mu$ is compactly supported and has density $q(x) \in C^1(\RR^n)$ with respect to $\cL_n$, the Lebesgue measure.
  In this case, for a fixed $i,j$ pair, applying integration by parts twice,
  \begin{align*}
    \iint \partial_{x_i}\partial_{y_j} K(x,y)\dd\mu(x)\dd\mu(y) &=\iint \partial_{x_i}\partial_{y_j} K(x,y)q(x )q(y)\dd x \dd y  \\
                                                                &= \iint K(x, y) \partial_{i} q(x) \partial_{j} q(y) \dd x \dd y.
  \end{align*}
  Hence
  \begin{align*}
    \sum_{i,j\in [n]}\iint \partial_{x_i}\partial_{y_j} K(x,y)\dd\mu(x)\dd\mu(y) = \iint K(x, y) (\div  q)(x) (\div q)(y) \dd x \dd y.
  \end{align*}
  Define a signed measure $\nu$ via $\dd\nu(x) \defeq \div q(x)\dd x$. Since $q \in C^1(\RR^n)$ vanishes outside a compact set, we see that $\nu$ is finite.
  Hence $K$ being i.s.p.d. implies the desired inequality.

  Now suppose $\mu$ is a general finite signed measure.
  Let $\{\zeta_\eps\}_{\eps}$ be a family of compactly supported smooth mollifier satisfying \cref{defn:mollifiers}.
  Then the measure $\zeta_\eps * \mu$ defined as, for a Borel $B \subset \RR^n$,
  \begin{align*}
    (\zeta_\eps * \mu)(B) \defeq \int_B \int \zeta(x-y) \dd\mu(y) \dd x,
  \end{align*}
  has density $q_\eps(y) \defeq \int \zeta(x-y) \dd\mu(y)$.

  Define a compactly supported finite measure $\nu_\eps$ by $\nu_\eps(A) = (\zeta_\eps * \mu)(A \cap B_{1/\eps}(0))$, where $B_{1/\eps}(0)$ is the ball with radius $1/\eps$ centered at $0$.
  We next show that $\nu_\eps \to \mu$ in weak convergence. 
  For any bounded continuous function $f$, 
  \begin{align*}
    \int f \dd\nu_\eps &= \int f(x) 1_{B_{1/\eps}(0)}(x) \int \zeta_\eps(x-y)\dd\mu(y) \dd x \\
                       &= \int \left( \int f(x) 1_{B_{1/\eps}(0)}(x) \zeta_\eps(x-y)\dd x \right) \dd\mu(y),
  \end{align*}
  where we used Fubini's theorem and H\"{o}lder's inequality that for any $y$,
  \[
    \abs{\int f(x) 1_{B_{1/\eps}(0)}(x) \zeta_\eps(x-y)\dd x} \le \norm{f}_\infty
  .\]
  Applying dominated convergence theorem, we obtain
  \begin{align*}
    \lim_{\eps \to 0} \int f \dd\nu_\eps &= \int \lim_{\eps \to 0}\left( \int f(x) 1_{B_{1/\eps}(0)}(x) \zeta_\eps(x-y)\dd x \right) \dd\mu(y) \\
                                         &= \int \lim_{\eps \to 0}\left(f \cdot 1_{B_{1/\eps}(0)} * \zeta_\eps(y) \right) \dd\mu(y) 
                                         = \int f(y) \dd\mu(y),
  \end{align*}
  where we used the fact that $\zeta_\eps$ is even and \cref{prop:conv_pw_conv_ex} (the set of discontinuous points of the function $f(x) \cdot 1_{B_{1/\eps}(0)}(x)$ has measure zero so the conclusion of \cref{prop:conv_pw_conv_ex} still holds a.e.).

  Finally, previous results show that $\lim_{\eps \to 0} \nu_\eps \times \nu_\eps = \mu \times \mu$ weakly.
  Since $\sup_{x,y} \abs{\partial_{x_i}\partial_{y_j} K(x,y)} < \infty$, we have
  \begin{align*}
   \sum_{i,j\in [n]}\iint \partial_{x_i}\partial_{y_j} K(x,y)\dd\mu(x)\dd\mu(y) = \lim_{\eps \to \infty} \sum_{i,j\in [n]}\iint \partial_{x_i}\partial_{y_j} K(x,y)\dd\nu_\eps(x)\dd\nu_\eps(y) \ge 0.
  \end{align*}
\end{proof}

\begin{proposition}\label{prop:wgf_lambda_disp_cvx}
  For each $\eps > 0$, the function $\cE_\eps$ is $\lambda_\eps$-convex along generalized geodesics, where 
  \[
    \lambda_\eps = -2 \sup_{x,y\in\RR^n}\norm{\hess_1 W_\eps(x,y)}_2 > -\infty
  ,\]
  where we use $\hess_i W_\eps$ to denote the Hessian of $W_\eps$ with respect to the $i$th input.
\end{proposition}
\begin{proof}
  Let $\{\mu_t^{2\to 3}\}_{t \in [0, 1]}$ be a generalized geodesic corresponding to $\bm\gamma \in \cP_2((\RR^n)^3)$ with base $\mu_1 \in \cP_2(\RR^n)$ connecting $\mu_2, \mu_3\in\cP_2(\RR^n)$.
  By \citet[Lemma 2.7]{craig2022blob}, it suffices to show that 
  \[
    \cE_\eps(\mu_3) - \cE_\eps(\mu_2) - \dv{}{t}\bigg|_{t=0}\cE_\eps(\mu_t^{2\to 3}) \ge \frac{\lambda_\eps}{2}W^2_{2,\bm\gamma}(\mu_2,\mu_3)
  .\]
  We compute, using \cref{lem:wgf_energy_dt},
  \begin{align*}
    &\cE_\eps(\mu_3) - \cE_\eps(\mu_2) - \dv{}{t}\bigg|_{t=0}\cE_\eps(\mu_t^{2\to 3}) \\
    =& \iint W_\eps(z,z')\dd\mu_3(z)\dd\mu_3(z') - \iint W_\eps(y,y')\dd\mu_2(y)\dd\mu_2(y') - \dv{}{t}\bigg|_{t=0}\cE_\eps(\mu_t^{2\to 3}) \\
    =& \iint \dd\bm\gamma(x',y',z')\dd\bm\gamma(x,y,z) (W_\eps(z,z')-W_\eps(y,y') \\
     &\hspace*{1.5in} -\nabla_1 W_\eps(y,y')^\top(z-y)-\nabla_2 W_\eps(y,y')^{\top}(z'-y')). \numberthis\label{eqn:wgf_cvx_pf_tangent_exp}
  \end{align*}
  By the integral form of Taylor's theorem, we have
  \begin{align*}
    W_\eps(z,z') = W_\eps(y, y') + \begin{pmatrix}\nabla_1 W_\eps(y,y')\\ \nabla_2 W_\eps(y,y')\end{pmatrix}^\top \begin{pmatrix} z-y\\z'-y' \end{pmatrix} + \\ 
    \int_0^1 (1-t)\begin{pmatrix} z-y\\ z'-y'\end{pmatrix}^\top 
    \begin{pmatrix} 
      \hess_1 W_\eps& \nabla_2\nabla_1 W_\eps\\ 
      \nabla_1\nabla_2 W_\eps & \hess_2 W_\eps \\ 
    \end{pmatrix}\bigg|_{(z+t(y-z),z'+t(y'-z'))}
    \begin{pmatrix} z-y\\ z'-y'\end{pmatrix} \dd t.\numberthis\label{eqn:wgf_cvx_pf_taylor_remainder}
  \end{align*}
  We use $\nabla_1 \nabla_2 W_\eps$ to denote the matrix $\nabla_x \nabla_y W_\eps(x,y)$.
  Note the integrand in \eqref{eqn:wgf_cvx_pf_tangent_exp} is precisely \eqref{eqn:wgf_cvx_pf_taylor_remainder}.

  We next show that the terms involving $\nabla_2 \nabla_1 W_\eps, \nabla_1 \nabla_2 W_\eps$ can be ignored when lower bounding \eqref{eqn:wgf_cvx_pf_tangent_exp}.
  That is, we want to show
  \begin{align*}
    \iint \left( \sum_{i,j\in [n]} \int_0^1 (1-t) \partial_{1,i}\partial_{2,j} W_\eps(z+t(y-z), z'+t(y'-z')) \dd t(z_{i}-y_{i})(z'_{j}-y'_{j}) \right) & \\
    \dd\bm\gamma(x',y',z')\dd\bm\gamma(x,y,z) & \ge 0, 
  \end{align*}
  where we use $\partial_{1,i}\partial_{2,j}W_\eps$ to denote $\partial_{x_i}\partial_{y_j} W_\eps(x, y)$.
  Fix $i,j\in [n]$ and $t \in [0, 1)$.
  Let $\bm h$ be the map $(x,y,z) \mapsto (x,y, z+t(y-z))$. Let $\hat{\bm\gamma} \defeq \pi^{2, 3}_\# \bm h_\#\bm\gamma$.
  Then after applying Fubini's theorem (by \cref{ass:wgf}, $\partial_{1,i}\partial_{2,j} W_\eps$ are bounded),
  \begin{align*}
    & \iint \partial_{1,i}\partial_{2,j} W_\eps(z+t(y-z), z'+t(y'-z')) (z_{i}-y_{i})(z'_{j}-y'_{j})\dd\bm\gamma(x',y',z')\dd\bm\gamma(x,y,z) \\
    =& \iint \partial_{1,i}\partial_{2,j} W_\eps(z,z') \frac{(z_i-y_i)(z'_j-y'_j)}{(1-t)^2}\dd\hat{\bm\gamma}(y,z)\dd\hat{\bm\gamma}(y',z').\numberthis \label{eqn:wgf_cvx_pf_cov}
  \end{align*}
  Define a signed measure $\eta$ via, for Borel $B \subset \RR^n$,
  \[
    \eta(B) \defeq \int_{z\in B} (z_i-y_i)\dd\hat{\bm\gamma}(y,z) 
  .\]
  Note that 
  \begin{align*}
    \eta(\RR^n) &= \int (z_i - y_i)\dd\hat{\bm\gamma}(y,z) = \int (z_i+t(y_i-z_i)-y_i) \dd\bm\gamma(x,y,z) \\
                &\le 2(M_1(\mu_2) + M_1(\mu_3)) \le 2(M_2(\mu_2) + M_2(\mu_3)) < \infty,
  \end{align*}
  where $M_i(\mu)$ indicates the $i$th moment of $\mu$, so $\eta$ is a finite measure.
  Then \eqref{eqn:wgf_cvx_pf_cov} becomes
  \begin{align*}
    (1-t)^{-2} \iint \partial_{1,i}\partial_{2,j} W_\eps(z,z')\dd\eta(z)\dd\eta(z') \ge 0,
  \end{align*}
  where we applied \cref{lem:mix_diff_kernel_ispd} while noticing that $W_\eps$ is i.s.p.d. on any compact set.

  Now plugging \eqref{eqn:wgf_cvx_pf_taylor_remainder} into \eqref{eqn:wgf_cvx_pf_tangent_exp} while discarding $\nabla_2\nabla_1 W_\eps, \nabla_1\nabla_2 W_\eps$ terms, we have
  \begin{align*}
    &\cE_\eps(\mu_3) - \cE_\eps(\mu_2) - \dv{}{t}\bigg|_{t=0}\cE_\eps(\mu_t^{2\to 3}) \\
    \ge& \iint \int_0^1(1-t) 
    \begin{pmatrix} z-y\\ z'-y'\end{pmatrix}^\top 
    \begin{pmatrix} 
      \hess_1 W_\eps& 0\\ 
      0 & \hess_2 W_\eps \\ 
    \end{pmatrix}\bigg|_{(z+t(y-z),z'+t(y'-z'))}
    \begin{pmatrix} z-y\\ z'-y'\end{pmatrix} 
    \dd t\\
       & \hspace*{3in} \dd\bm\gamma(x',y',z')\dd\bm\gamma(x,y,z) \\
    \ge& -\frac{1}{2} \iint \left( \norm{z-y}^2_2 \sup_{x,y}\norm{\hess_1 W_\eps(x,y)}_2 + \norm{z'-y'}^2_2 \sup_{x,y}\norm{\hess_2 W_\eps(x,y)}_2 \right)\\
       & \hspace*{3in} \dd\bm\gamma(x',y',z')\dd\bm\gamma(x,y,z) \\
    =& -\sup_{x,y\in\RR^n}\norm{\hess_1 W_\eps(x,y)}_2 W^2_{2,\bm\gamma}(\mu_2,\mu_3).
  \end{align*}
  \cref{ass:wgf} makes sure 
  \[
    \lambda_\eps \defeq -2 \sup_{x,y\in\RR^n}\norm{\hess_1 W_\eps(x,y)}_2 > -\infty.
  \]

\end{proof}

\begin{proposition}\label{prop:wgf_min_norm_subdiff}
  For $\mu \in D(\abs{\cE_\eps})$, the min-norm subdifferential $\partial^\circ \cE_\eps(\mu)$ is given by
  \[
    \partial^\circ \cE_\eps(\mu)(x) = 2\nabla_x \left(\int W_\eps(x,y)\dd\mu(y) \right)
  .\]
\end{proposition}
\begin{proof}
  Fix $\mu \in D(\abs{\cE_\eps})$ and $\nu \in \cP_2(\RR^n)$.
  For any $\bm\gamma \in \Gamma_o(\mu, \nu)$, consider the generalized geodesic $\{\mu_t\}_{t\in[0, 1]}$ connecting $\mu$ to $\nu$ with base $\mu$ with associated plan $\hat{\bm\gamma} \in \cP_2((\RR^n)^3)$ such that $\pi^{1,3}_\#\hat{\bm\gamma} = \pi^{2,3}_\#\hat{\bm\gamma} = \bm\gamma$.
  By \cref{prop:wgf_lambda_disp_cvx}, we have
  \begin{align*}
    \cE_\eps(\nu) - \cE_\eps(\mu) &\ge \dv{t}\bigg|_{t=0} \cE_\eps(\mu_t) + \frac{\lambda_\eps}{2} W^2_2(\mu, \nu) \\
                                  &= 2\iint \nabla_1 W_\eps(y,y')^\top (z-y)\dd\mu(y')\dd\hat{\bm\gamma}(x,y,z)+ \frac{\lambda_\eps}{2} W^2_2(\mu, \nu) \\
                                  &= 2 \int \left(\int \nabla_1 W_\eps(y,y') \dd\mu(y') \right)^\top (z-y) \dd\bm\gamma(y,z) +  \frac{\lambda_\eps}{2} W^2_2(\mu, \nu).
  \end{align*}
  This proves $\bm w_\eps(x) \defeq 2 \int \nabla_1 W_\eps(x,y) \dd\mu(y) \in \partial \cE_\eps(\mu)$.

  To show that $\bm w_\eps(x) = \partial^\circ \cE_\eps(\mu)$, we follow the argument in \citet[Proposition 3.8]{craig2022blob}.
  By \cref{prop:min_norm_subdiff}, it suffices to show $\abs{\partial\cE_\eps}(\mu) \ge \norm{\bm w_\eps(x)}_{L^2(\mu)}$.
  Fix $\bm\xi \in L^2(\mu;\RR^n)$ with $\norm{\bm\xi}_{L^2(\mu)} > 0$, and let $\mu_t \defeq (\bm I + t \bm\xi)_\# \mu$.
  By the definition of local slope $\abs{\partial\cE_\eps}$, we have
  \begin{align*}
    \abs{\partial\cE_\eps}(\mu) &= \limsup_{\nu \to \mu} \frac{(\cE_\eps(\mu) - \cE_\eps(\nu))_+}{W_2(\mu, \nu)} 
                                \ge \limsup_{t \to 0} \frac{(\cE_\eps(\mu) - \cE_\eps(\mu_t))_+}{W_2(\mu, \mu_t)} \\
                                &\ge \limsup_{t \to 0} \frac{\cE_\eps(\mu_t) - \cE_\eps(\mu)}{t\norm{\bm\xi}_{L^2(\mu)}} 
                                = \norm{\bm\xi}_{L^2(\mu)}^{-1} \dv{}{t}\bigg|_{t=0}\cE_\eps(\mu_t).
  \end{align*}
  By \cref{lem:wgf_energy_dt} applied to $\bm\gamma \defeq (\bm I, \bm I, \bm I + \bm\xi)_\# \mu$, we get
  \begin{align*}
    \dv{}{t}\bigg|_{t=0}\cE_\eps(\mu_t) &= 2 \iint \nabla_1 W_\eps(y,y')^\top (z-y)\dd\mu(y')\dd\bm\gamma(x,y,z) \\
                                        &= 2 \iint \nabla_1 W_\eps(y,y')^\top \bm\xi(y)\dd\mu(y')\dd\mu(y) \\
                                        &= \iint \bm w_\eps(y)^\top \bm\xi(y) \dd\mu(y).
  \end{align*}
  By taking $\bm\xi = \bm w_\eps$, we have
  \begin{align*}
    \abs{\partial\cE_\eps}(\mu) \ge \norm{\bm\xi}_{L^2(\mu)}^{-1} \dv{}{t}\bigg|_{t=0}\cE_\eps(\mu_t) = \norm{\bm\xi}_{L^2(\mu)}^{-1} \norm{\bm\xi}_{L^2(\mu)}^{2} = \norm{\bm\xi}_{L^2(\mu)}.
  \end{align*}
\end{proof}
Thanks to \cref{prop:wgf_lambda_disp_cvx}, we can now apply \cref{thm:wgf_exist_unique} to conclude the existance and uniqueness of the Wasserstein gradient flow $\mu_t \in \AC_\loc^2((0, T); \cP_2(\RR^n))$ of $\cE_\eps$ with the velocity field $-\partial^\circ\cE_\eps(\mu_t)$ whose form is given by \cref{prop:wgf_min_norm_subdiff}.



==> math_commands.tex <==

\usepackage{amsmath,amsfonts,bm}

\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

\newcommand{\newterm}[1]{{\bf #1}}


\def\figref#1{figure~\ref{#1}}
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
\def\secref#1{section~\ref{#1}}
\def\Secref#1{Section~\ref{#1}}
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
\def\eqref#1{equation~\ref{#1}}
\def\Eqref#1{Equation~\ref{#1}}
\def\plaineqref#1{\ref{#1}}
\def\chapref#1{chapter~\ref{#1}}
\def\Chapref#1{Chapter~\ref{#1}}
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
\def\algref#1{algorithm~\ref{#1}}
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
\def\partref#1{part~\ref{#1}}
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

\newcommand{\pdata}{p_{\rm{data}}}
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} %

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} %


\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}

\let\ab\allowbreak
